Optimized Spatial Architecture Mapping Flow for Transformer Accelerators

Recent innovations in Transformer-based large language models have significantly advanced the field of general-purpose neural language understanding and generation. With billions of trainable parameters, deployment of these large models relies on high-performance hardware accelerators to efficiently deliver the required computation. Spatial architectures, such as TPUs, offer a promising solution to accelerating computation-intensive workloads. However, the design process for existing spatial architectures is predominantly manual, and it often involves time-consuming redesigns for new applications and new problem dimensions, which greatly limits the development of optimally designed accelerators for Transformer models. To address these challenges, we propose SAMT (Spatial Architecture Mapping for Transformers), a comprehensive framework designed to optimize the dataflow mapping of Transformer inference workloads onto spatial accelerators. We demonstrate the effectiveness of SAMT in improving the performance of spatial accelerators for Transformer models. We propose and leverage the dynamic operator fusion schemes for the Transformer models and co-search the optimal dataflow mapping strategies for spatial accelerators. SAMT significantly reduces inference latency by 12% to 91% and energy consumption by 3% to 23% for evaluated Transformer models compared to traditional spatial accelerator designs among edge, mobile and cloud settings.

==> Sections/03_Motivation.tex <==
\section{Challenges of the Transformer Accelerator}

\label{sec:motivation}

There has been a focus on making transformer models more efficient in both industry and academia recently. Identifying the bottlenecks in the existing transformer model and understanding the limits of current hardware support for transformer model will be crucial. \cite{kim2023stack,kao2023flat}


\subsection{Low Arithmetic Intensity for Longer Sequence}

With the recent trend of ChatGPT, people are expecting longer input and output from those LLMs(large language models). However, there are limits to the sequence length of LLMs. For example, the token limit for GPT-35-Turbo is 4k, GPT-4 is 8k and GPT-4-32-k is 32k. To understand the reason behind the limits of tokens, we profiled the arithmetic intensity $I$, which is calculated by dividing FLOPs (the number of floating-point operations) by MOPs (the number of memory access counts) (assuming that each memory access will fetch one-byte data):

\begin{equation}
    I = \frac{FLOPs}{MOPs}
\end{equation}

 As shown in Fig. \ref{fig:Arithmetic Intensity}(a), the arithmetic intensity first increases then decreases after reaching sequence length $l$ = 512 for both BERT-Base model and the GPT3-Medium model. The main reason for this drop in arithmetic intensity is that some operations' (like $A = Q \otimes K$ and $S = Softmax (A)$) memory access count will scale up quadratically with the sequence lengths $l$ while keeping the number of floating point operations at low level. In Fig. \ref{fig:Arithmetic Intensity}(b), we can see that those operations will quickly dominate in memory access count in the entire transformer model as sequence length $l$ increases. 

As shown in Fig. \ref{fig:Arithmetic Intensity}(c), we can find some operators have low arithmetic intensity. As sequence length increases, Operator $QKVY$ (projection) and $MLP$'s (feed-forward) arithmetic intensity increases accordingly while the other two type operators $A/O$ and $S$'s arithmetic intensity stay steady or even decreases. This further proves that those memory operations will become a bottleneck when sequence length increases in the transformer model.

%Quantify the operators
%Transformer vs CNN

%Most of the large language model 

%\subsection{Current CNN accelerators for transformer}
%Pros/Cons 
%SOTA Throughput/energy
%As with CNNs, the majority of cycles for transformer models are spent on GEMM or GEMV (matrix-vector multiplication). We can try to leverage the current CNN accelerators like TPU, Eyeriss, and NVDLA\cite{jouppi2023tpu,eyeriss,NVDLA} to accelerate the transformer model. However, due to the prohibitively large intermediate tensors for operators like $O$ and $S$, which quadratically scale with the sequence length $l$, those accelerators do not have enough on-chip memory $S2$ to store all of the intermediate tensors. That will incur a lot of memory read/write from the off-chip memory $S3$ as we described in Fig.\ref{fig:spatial arch}.

%Even if we can customize some hardware configurations (number of PEs, $S2$ size, NoCs) and adapt those accelerator architecture design methodologies (the dataflow type), it is still hard for us to find the optimal accelerators without trying out all the combinations of hardware configurations and different transformer models. This time-consuming process needs to be necessitated. 

\subsection{Lack of fusion exploration in flexible dataflow accelerator }

There are several hardware-aware compiler frameworks for fusion optimization. TVM \cite{chen2018tvm}, for instance, leverages deep learning models to determine efficient fusion strategies. It optimizes fusion based on the target hardware's cache size and memory hierarchy, but it works on a fixed dataflow and doesn't consider various possible dataflows. XLA \cite{xla}, another compiler, is primarily optimized for CPU and GPU backends supported by LLVM. Although XLA can be adapted to non-CPU-like hardware that lacks an existing LLVM backend, this adaptation requires significant effort to implement a new backend for the desired hardware. Therefore, XLA does not directly target flexible spatial accelerators. FLAT\cite{kao2023flat} tries to target flexible accelerators and perform inter-layer fusion; however, it is limited to activation-to-activation fusion and does not fully explore all the fusion schemes. Removing this restriction brings more fusion possibilities at the cost of larger intermediate storage.
%The previous concern about performance loss when fusing fully connected layers has been addressed by the most recent work \cite{liu2023blockwise}. \FT{This explanation does not fit in this section's context} \cite{liu2023blockwise} presents a block-wise parallel transformer for GPU work that shows the fusion entire attention block and feed-forward layer does not lose any performance. 

%There are several compiler frameworks that specialize in optimizing different aspects of hardware and software interaction. TVM, for instance, leverages deep learning models to determine efficient fusion strategies. It optimizes fusion based on the target hardware's cache size and memory hierarchy. XLA, another compiler, is primarily optimized for CPU and GPU backends supported by LLVM. Although XLA can be adapted to non-CPU-like hardware that lacks an existing LLVM backend, this adaptation requires significant effort to implement a new backend for the desired hardware. Therefore, XLA does not directly target spatial accelerators as effectively.FLAT\cite{kao2023flat} tried to perform inter-layer fusion; however, it only limited to activation-to-activation fusion and did not fully explore the fusion scheme. The previous concern about performance loss when fusing fully connected layers has been addressed by the most recent work \cite{liu2023blockwise}. \cite{liu2023blockwise} presented a blockwise parallel transformer for GPU work that shows the fusion entire attention block and feedforward layer does not lose any performance. 

%There are some existing compiler works like TVM
%TVM used deep learning model to find the efficient fusion. SAMT iterate through entire fusion-scheme while considering different dataflows (computation order, tile size etc). TVM can perform fusion optimization on the target hardware considering cache size and memory hierarchy. SAMT can optimize the fusion considering number of PEs, NoC, S1, S2, Offchip bandwidth. Additionally, SAMT can be applied to more flexible spatial accelerators as well (like considering different dataflow for each operators). 
%XLA is optimzed for CPU and GPU backends that could be supported by LLVM. Even though it supports non-cpu-like hardware without an existing LLVM backend, that requires a new implementation of backend for XLA on the desired hardware, which requires a lot of effort. Hence, XLA does not directly target the spatial accelerator like SAMT does. There are also other compiler works that include optimization of operators like Ansor and AMOS. 

% GPU reduce kernel overhead
%FLAT\cite{kao2023flat} tried to perform inter-layer fusion; however, it only limited to activation-to-activation fusion and did not fully explore the fusion scheme. The previous concern about performance loss when fusing fully connected layers has been addressed by the most recent work \cite{liu2023blockwise}. \cite{liu2023blockwise} presented a blockwise parallel transformer for GPU work that shows the fusion entire attention block and feedforward layer does not lose any performance. 

%\subsection{Lack of flexible dataflow exploration}

Contrary to all works that mainly focus on searching for appropriate fusion scheme for a fixed dataflow, to the best of our knowledge, there is no prior work that removes all limitations on the dataflow as it wants to search for optimal fusion. Despite increasing the design search space, it brings great optimization opportunities. This is evident that underlying hardware must support the output of such framework. The goal of this work is to introduce such framework that finds the best fusion scheme with arbitrary dataflow to be exploited by a flexible hardware accelerator.

%Previous work also did not consider the impact of the refill and decoding stage when inferring the decoder-only transformer model like (GPT-3). In the prefill stage, prompt processing can be parallelized since all the inputs (the prompt) are given. However, in the decoding phase, only one token will be generated at a time. This autoregressive processing can not be parallelized due to data dependency thus we can not model the processing the same way as the encoder-only transformer model. 

